A Correlation-Breaking Interleaving of Polar Codes in Concatenated Systems

It is known that the bit errors of polar codes with successive cancellation (SC) decoding are coupled. However, existing concatenation schemes of polar codes with other error correction codes rarely take this coupling effect into consideration. To achieve a better error performance of concatenated systems with polar codes as inner codes, one can divide all bits in an outer block into different polar blocks to completely de-correlate the possible coupled errors in the transmitter side. We call this interleaving a blind interleaving (BI) which serves as a benchmark. Two BI schemes, termed BI-DP and BI-CDP, are proposed in the paper. To better balance performance, memory size, and the decoding delay from the de-interleaving, a novel interleaving scheme, named the correlation-breaking interleaving (CBI), is proposed. The CBI breaks the correlated information bits based on the error correlation pattern proposed and proven in this paper. The proposed CBI scheme is general in the sense that any error correction code can serve as the outer code. In this paper, Low-Density Parity-Check (LDPC) codes and BCH codes are used as two examples of the outer codes of the interleaving scheme. The CBI scheme 1) can keep the simple SC polar decoding while achieving a better error performance than the state-of-the-art (SOA) direct concatenation of polar codes with LDPC codes and BCH codes; 2) achieves a comparable error performance as the BI-DP scheme with a smaller memory size and a shorter decoding delay. Numerical results are provided to verify the performance of the BI schemes and the CBI scheme.

==> ref_polar_tc18 <==
% Encoding: UTF-8
@book{lin_ecc04,
author = {Shu Lin and Daniel J. Costello},
title={Error Control Coding},
publisher = {Pearson Prentice Hall},
year={2004},
edition={2nd}
}

@InProceedings{effros_isit10,
  author    = {M. Bakshi and S. Jaggi and M. Effros},
  title     = {Concatenated Polar codes},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2010},
  pages     = {918-922},
  month     = jun,
}

@Article{song_el17,
  author  = {J. Park and I. Kim and H. Song},
  title   = {Construction of parity-check-concatenated polar codes based on minimum Hamming weight codewords},
  journal = {Electron. Lett.},
  year    = {2017},
  volume  = {53},
  number  = {14},
  pages   = {924-926},
  month   = jul,
}

@Article{jiang_cl16,
  author  = {T. Wang and D. Qu and T. Jiang},
  title   = {Parity-Check-Concatenated Polar Codes},
  journal = {IEEE Commun. Lett.},
  year    = {2016},
  volume  = {20},
  number  = {12},
  pages   = {2342-2345},
  month   = dec,
}
@misc{abbe_stoc15,
  author = {Emmanuel Abbe and Amir Shpilka and Avi Wigderson},
  title = "{Reed-Muller codes for random erasures and errors}",
  howpublished = "\url{http://www.princeton.edu/~eabbe/publications/RM-arxiv3.pdf}",
  year = {2015}
}

@Article{arikan_icl08,
  author  = {Ar$\i$kan, E.},
  title   = {{A performance comparison of polar codes and reed-muller codes}},
  journal = {IEEE Commun. Lett.},
  year    = {2008},
  volume  = {12},
  number  = {6},
  pages   = {447-449},
  month   = jun,
}

@Article{arikan_icl11,
  author  = {Ar$\i$kan, E.},
  title   = {{Systematic polar coding}},
  journal = {IEEE Commun. Lett.},
  year    = {2011},
  volume  = {15},
  number  = {8},
  pages   = {860-862},
  month   = aug,
}

@InProceedings{arikan_isit09,
  author    = {Ar$\i$kan, E. and Telatar, I.E.},
  title     = {{On the Rate of Channel Polarization}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2009},
  pages     = {1493-1495},
}

@Article{arikan_iti09,
  author  = {Ar$\i$kan, E.},
  title   = {{Channel polarization: A method for constructing capacity-achieving codes for symmetric binary-input memoryless channels}},
  journal = {IEEE Trans. Inf. Theory},
  year    = {2009},
  volume  = {55},
  number  = {7},
  pages   = {3051-3073},
  month   = jul,
}

@InProceedings{barron_isit11,
  author    = {Abbe, E. and Barron, A.},
  title     = {{Polar Coding Schemes for the AWGN Channel}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2011},
  pages     = {194-198},
}

@InProceedings{barry_icc13,
  author =    {Ubaid U. Fayyaz and John R. Barry},
  title =     {{Polar codes for partial response channels}},
  booktitle = {Proc. IEEE International Conference on Communications (ICC)},
  year =      {2013},
  pages =     {4337 - 4341}
}

@Article{C.Wu_10,
  author =  {C. Wu and J. Cruz},
  title =   {{RS plus LDPC codes for perpendicular magnetic recording}},
  journal = {IEEE Transactions on Magnetics},
  year =    {2010},
  volume =  {46},
  number =  {16},
  pages =   {1416-1419}
}

@Article{C.Z_itcs14,
  author  = {C. Zhang and K. K. Parhi},
  title   = {{Latency analysis and architecture design of simplified SC polar decoders}},
  journal = {IEEE Trans. Circuits Syst. II, Exp. Briefs},
  year    = {2014},
  volume  = {61},
  pages   = {115-119},
  month   = feb,
}

@Article{C.Z_itsp13,
  author  = {C. Zhang and K. K. Parhi},
  title   = {{Low-latency sequential and overlapped architectures for successive cancellation polar decoder}},
  journal = {IEEE Trans. Signal Process.},
  year    = {2013},
  volume  = {61},
  pages   = {2429-2441},
  month   = may,
}

@techreport{channel_ieee_4a,
	title = "{IEEE 802.15.4a Channel Model - Final Report}",
	author = "Andreas F. Molisch and Kannan Balakrishnan 
		and Dajana Cassioli and Chia-Chin Chong and
		Shahriar Emami and Andrew Fort and Johan Karedal and
		Juergen Kunisch and Hans Schantz and Ulrich Schuster 
		and Kai Siwiak",
	institution = "IEEE 802.15 TG4a",
	year = "2004"
	}

@Article{E.M_06,
  author =  {E. M. Kurtas and A. Kuznetsov and I. Djurdjevic},
  title =   {{System perspectives for the application of structured LDPC codes to data storage devices}},
  journal = {IEEE Transactions on Magnetics},
  year =    {2006},
  volume =  {42},
  number =  {2},
  pages =   {200-207}
}
@INPROCEEDINGS{eslami_allerton10, 
author={Eslami, A. and Pishro-Nik, H.}, 
booktitle={48th Annual Allerton Conference on Communication, Control, and Computing (Allerton)}, 
title="{On Bit Error Rate Performance of Polar Codes in Finite Regime}", 
year={2010}, 
pages={188-194}, 
}

@InProceedings{eslami_isit11,
  author    = {A. Eslami and H. Pishro-Nik},
  title     = {{A practical approach to polar codes}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2011},
  pages     = {16-20},
  month     = jul,
}

@Article{G.Sarkis_16,
  author =  {G. Sarkis, I. Tal, P. Giard, A. Vardy, C. Thibeault, and W. J. Gross},
  title =   {{Flexible and Low-Complexity Encoding and Decoding of Systematic Polar Codes}},
  journal = {IEEE Transactions on Communication},
  year =    {2016},
  volume =  {64},
  number =  {7},
  pages =   {2732–2745},
  month =   {June}
}

@InProceedings{guo_isit14,
  author    = {Jing Guo and Minghai Qin and Albert Guillen i Fabregas and Paul H. Siegel},
  title     = {{Enhanced belief propagation decoding of polar codes through concatenation}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2014},
  pages     = {2987 - 2991},
  month     = jun,
}

@Article{H.M_11,
  author =  {H. Mahdavifar and A. Vardy},
  title =   {{Achieving the Secrecy Capacity of Wiretap Channels Using Polar Codes}},
  journal = {IEEE Trans. Inf. Theory},
  year =    {2011},
  volume =  {57},
  number =  {10},
  pages =   {6428–6443},
  month =   oct
}

@Article{hassani_iti13,
  author =  {Hassani, S.H. and Mori, R. and Tanaka, T. and Urbanke, R.L.},
  title =   {{Rate-dependent analysis of the asymptotic behavior of channel polarization}},
  journal = {IEEE Trans. Inf. Theory},
  year =    {2013},
  volume =  {59},
  number =  {4},
  pages =   {2267-2276}
}

@Article{hong_icl16,
  author  = {H. Vangala and Y. Hong and E. Viterbo},
  title   = {{Efficient algorithms for systematic polar encoding}},
  journal = {IEEE Commun. Lett.},
  year    = {2016},
  volume  = {20},
  number  = {1},
  pages   = {17-20},
  month   = jan,
}
@misc{ido_15,
  author = {Gabi Sarkis and Ido Tal and Pascal Giard and Alexander Vardy and
Claude Thibeault and Warren J. Gross},
  title = "{Flexible and Low-Complexity Encoding and
Decoding of Systematic Polar Codes}",
  howpublished = "Online: \url{http://arxiv.org/abs/1507.03614v2}", 
}
@inproceedings{jonward_mil07,
	author = "Jon R. Ward and J. Keith Townsend",
	title = "{Chip Discrimination for UWB Impulse Radio Networks in Multipath Channels}",
	booktitle = "{IEEE Military Communications Conference (MILCOM)}",
	pages = "1-6",
	month = "Oct.",
	year = "2007"
	}
@article{kaufman_it12,
	author={Tali Kaufman and Shachar Lovett and Ely Porat}, 
	journal={IEEE Transactions on Information Theory}, 
	title="{Weight Distribution and List-Decoding Size of Reed-Muller Codes}", 
	year={2012}, 
	month={May}, 
	volume={58}, 
	number={5}, 
	pages={2689-2696}
}
@ARTICLE{korada_iti10, 
author={Satish Babu Korada and Eren Sasoglu and R��diger Urbanke}, 
journal={IEEE Transactions on Information Theory}, 
title="{Polar Codes: Characterization of Exponent, Bounds, and Constructions}", 
year={2010}, 
month={December}, 
volume={56}, 
number={12}, 
pages={6253-6264}
}
@book{levy_detection08,
	author = "Bernard C. Levy",
	title = "{Priciples of Signal Detection and Parameter Estimation}",
	publisher = "Springer",
	year = "2008"
	}

@Misc{li_jsac15,
  author =       {Liping Li and Wenyi Zhang and Yanjun Hu},
  title =        {{On the error performance of systematic polar codes}},
  howpublished = {[Online]. Available: \url{http://arxiv.org/abs/1504.04133}},
  year =         {2015}
}

@InProceedings{li_socc15,
  author    = {Liping Li and Wenyi Zhang},
  title     = {{On the encoding complexity of systematic polar codes}},
  booktitle = {Proc. IEEE Int. Syst.-on-Chip Conf. (SOCC)},
  year      = {2015},
  pages     = {508-513},
  month     = sep,
}

@Article{li_tvt18,
  author  = {L. Li and Z. Xu and Y. Hu},
  title   = {Channel Estimation With Systematic Polar Codes},
  journal = {IEEE Trans. Veh. Technol.},
  year    = {2018},
  volume  = {67},
  number  = {6},
  pages   = {4880-4889},
  month   = jun,
  issn    = {0018-9545},
  doi     = {10.1109/TVT.2018.2806364},
}
@Article{mori_icl09,
  author =   {R. Mori and T. Tanaka},
  title =    {{Performance of polar codes with the construction using density evolution}},
  journal =  {IEEE Commun. Lett.},
  year =     {2009},
  volume =   {13},
  number =   {7},
  pages =    {519--521},
  month =    jul,
  doi =      {10.1109/LCOMM.2009.090428},
  issn =     {1089-7798},
  keywords = {binary codes;computational complexity;decoding;binary erasure channel;capacity-achieving code construction method;decoding complexity;density evolution;linear complexity;low encoding complexity;polar codes;symmetric binary-input discrete memoryless channel;Arithmetic;Belief propagation;Linear code;Maximum likelihood decoding;Memoryless systems;Polarization;Statistics;Symmetric matrices;Channel polarization, polar codes, code construction, belief propagation, density evolution.}
}

@InProceedings{mori_isit09,
  author    = {Ryuhei Mori and Toshiyuki Tanaka},
  title     = {{Performance and Construction of Polar codes on Symmetric Binary-Input Memoryless Channels}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2009},
  pages     = {1496-1500},
  month     = {June},
}

@InProceedings{mori_isit10,
  author    = {Toshiyuki Tanaka and Ryuhei Mori},
  title     = {{Refined Rate of Channel Polarization}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2010},
  pages     = {889-893},
  month     = {June},
}
@INPROCEEDINGS{mori_itw10, 
author={Ryuhei Mori and Toshiyuki Tanaka}, 
booktitle={IEEE Information Theory Workshop (ITW)}, 
title="{Non-Binary Polar Codes using Reed-Solomon Codes and Algebraic Geometry Codes}", 
year={2010},  
pages={1-5}
}

@Article{niu_itc13,
  author  = {Kai Chen and Kai Niu and JiaRu Lin},
  title   = {{Improved successive cancellation decoding of polar codes}},
  journal = {IEEE Trans. Commun.},
  year    = {2013},
  volume  = {61},
  number  = {8},
  pages   = {3100-3107},
  month   = aug,
}

@InProceedings{park_isit13,
  author    = {Woomyoung Park and Alexander Barg},
  title     = {{Polar Codes for q-ary Channels, $q=2^r$}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2013},
  pages     = {955-969},
  month     = {Feb.},
}
@INPROCEEDINGS{pradhan_allerton11, 
author={Aria G. Sahebi and S. Sandeep Pradhan}, 
booktitle={2011 49th Annual Allerton Conference on Communication, Control, and Computing (Allerton)}, 
title="{Multilevel Polarization of Polar Codes Over Arbitrary Discrete Memoryless Channels}", 
year={2011}, 
month={September}, 
pages={1718-1725}
}
@book{proakis_digicom,
	author = "John G. Proakis",
	title  = "Digital Communications",
	publisher = "Mc Graw-Hill, Inc.",
	year = "2006",
	edition = "4th" 	}
@INPROCEEDINGS{q_bound_wu11, 
author={Mingwei Wu and Xuzheng Lin and Pooi-Yuen Kam}, 
booktitle={2011 IEEE 73rd Vehicular Technology Conference (VTC Spring)}, 
title={New Exponential Lower Bounds on the Gaussian Q-Function via Jensen's Inequality}, 
year={2011}, 
pages={1-5}, 
}
@misc{qiming_15,
  author = {Qiming Wang and Liping Li},
  title = "{On the Symmetry of Polar Codes for Symmetric Binary-Input Discrete Memoryless Channels}",
  howpublished = "\url{http://arxiv.org/abs/1504.04934}",
  year = {2015}
}
@misc{sasoglu_09,
  author = {Eren Sasoglu and Emre Telatar and Erdal Arikan},
  title = "{Polarization for Arbitrary Discrete Memoryless Channels}",
  howpublished = "Online: \url{http://arxiv.org/pdf/0908.0302v1.pdf}", 
}
@INPROCEEDINGS{sasoglu_itw10, 
author={Sasoglu, E. and Telatar, E. and Yeh, E.}, 
booktitle={ 2010 IEEE Information Theory Workshop (ITW)}, 
title="{Polar Codes for the Two-user Binary-Input Multiple-Access Channel}", 
year={2010}, 
pages={1-5}, 
}
@INPROCEEDINGS{shi_icc12, 
author={Shi, Peng and Wenjuan Tang and Zhao, Shengmei and Wang, Bei}, 
booktitle={2012 IEEE 14th International Conference on Communication Technology (ICCT)}, 
title="{Performance of Polar Codes on Wireless Communication Channels}", 
year={2012}, 
pages={1134-1138}, 
}
@INPROCEEDINGS{tal_icassp11, 
author={C. Leroux and I. Tal and A. Vardy and W. J. Gross}, 
booktitle={2011 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
title="{Hardware Architectures for Successive Cancellation Decoding of Polar Codes}", 
year={2011}, 
pages={1665-1668}, 
month={May}
}

@Article{tanner_it04,
  author =  {R. Michael Tanner and Deepak Sridhara and Arvind Sridharan and Thomas E. Fuja and Daniel J. Costello},
  title =   {{LDPC block and convolutional codes based on circulant matrices}},
  journal = {IEEE Trans. Inf. Theory},
  year =    {2004},
  volume =  {50},
  number =  {12},
  pages =   {2966-2984},
  month =   {December}
}

@InProceedings{telatar_isit11,
  author    = {Pedarsani, R. and Hassani, S.H. and Tal, I. and Telatar, I.E.},
  title     = {{On the Construction of Polar Codes}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2011},
  pages     = {11-15},
}
@article{telatar_iti12,
author={E. Abbe and E. Telatar}, 
title="{Polar Codes for the m-User Multiple Access Channel}",
journal={IEEE Transactions on Information Theory},
volume=58,
number={8},
pages={5437�5448}, 
year={2012},
}
@INPROCEEDINGS{telatar_itw10, 
author={Abbe, E. and Telatar, I.E.}, 
booktitle={Information Theory and Applications Workshop (ITA)}, 
title="{MAC Polar Codes and Matroids}", 
year={2010}, 
month={Jan}, 
pages={1-8}, 
}

@Article{trifonov_itc12,
  author  = {Peter Trifonov},
  title   = {{Efficient design and decoding of polar codes}},
  journal = {IEEE Trans. Commun.},
  year    = {2012},
  volume  = {60},
  number  = {11},
  pages   = {3221-3227},
  month   = nov,
}

@InProceedings{urbanke_isit09,
  author    = {N. Hussami and S. Korada and R. Urbanke},
  title     = {{Performance of polar codes for channel and source coding}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2009},
  pages     = {1488-1492},
  month     = jun,
}

@InProceedings{urbanke_isit10,
  author    = {S. Hamed Hassani and R. Urbanke},
  title     = {{On the Scaling of Polar Codes: I. The Behavior of Polarized Channels}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2010},
  pages     = {874-878},
  month     = {June},
}

@Article{urbanke_iti14,
  author =  {S. Hamed Hassani and Kasra Alishahi and Rudiger Urbanke},
  title =   {{Finite-length scaling of polar codes}},
  journal = {IEEE Trans. Inf. Theory},
  year =    {2014},
  volume =  {60},
  number =  {10},
  pages =   {5875-5898},
  month =   {October}
}

@Article{urbanke_tc14,
  author =  {M. Mondelli and S. H. Hassani and R. L. Urbanke},
  title =   {{From polar to reed-muller codes: A technique to improve the finite-length performance}},
  journal = {IEEE Trans. Commun.},
  year =    {2014},
  volume =  {62},
  number =  {9},
  pages =   {3084-3091},
  month =   {Sept}
}
@Article{vangala_15,
  author =        {Vangala, Harish and Viterbo, Emanuele and Hong, Yi},
  title =         "{A Comparative Study of Polar Code Constructions for the AWGN Channel}",
  journal =       {arXiv preprint arXiv:1501.02473},
  year =          {2015}
}

@InProceedings{vardy_isit11,
  author    = {Tal, I. and Vardy, A.},
  title     = {{List Decoding of Polar Codes}},
  booktitle = {Proc. IEEE Int. Symp. Inform. Theory (ISIT)},
  year      = {2011},
  pages     = {1-5},
  month     = {July},
}

@ARTICLE{vardy_it02, 
author={Agrell, E. and Eriksson, T. and Vardy, A. and Zeger, K.}, 
journal={Information Theory, IEEE Transactions on}, 
title="{Closest Point Search in Lattices}", 
year={2002}, 
volume={48}, 
number={8}, 
pages={2201-2214},  
month={Aug}}
@ARTICLE{vardy_it03, 
author={Koetter, R. and Vardy, A.}, 
journal={Information Theory, IEEE Transactions on}, 
title="{Algebraic Soft-Decision Decoding of Reed-Solomon Codes}", 
year={2003}, 
volume={49}, 
number={11}, 
pages={2809-2825}, 
month={Nov}}

@Article{vardy_it13,
  author  = {Tal, I. and Vardy, A.},
  title   = {{How to construct polar codes}},
  journal = {IEEE Trans. Inf. Theory},
  year    = {2013},
  volume  = {59},
  number  = {10},
  pages   = {6562-6582},
  month   = oct,
}

@Article{vardy_it15,
  author =  {Tal, I. and Vardy, A.},
  title =   {{List decoding of polar codes}},
  journal = {IEEE Trans. Inf. Theory},
  year =    {2015},
  volume =  {61},
  number =  {5},
  pages =   {2213-2226},
  month =   {May}
}
@ARTICLE{vardy_iti11, 
author={Hessam Mahdavifar and Alexander Vardy}, 
journal={IEEE Transactions on Information Theory}, 
title="{Achieving the Secrecy Capacity of Wiretap Channels Using Polar Codes}", 
year={2011}, 
month={October}, 
volume={57}, 
number={10}, 
pages={6428-6443}
}

@Article{vardy_jsac14,
  author  = {Sarkis, G. and Giard, P. and Vardy, A. and Thibeault, C. and Gross, W.J.},
  title   = {{Fast polar decoders: Algorithm and implementation}},
  journal = {IEEE J. Sel. Areas Commun.},
  year    = {2014},
  volume  = {32},
  number  = {5},
  pages   = {946-957},
  month   = may,
}
@article{vishwanath_tc14,
  author = {Hongbo Si and Onur Ozan Koyluoglu and Sriram Vishwanath},
  journal={IEEE Transactions on Communications},
  title = "{Polar Coding for Fading Channels: Binary and Exponential Channel Cases}",
  year = {2014}, 
  month = {August},
  volume={62},
  number={8},
  pages={2638-2649}
}

@article{wei_it91,
	author={Victor K. Wei}, 
	journal={IEEE Transactions on Information Theory}, 
	title="{Generalized Hamming Weights for Linear Codes}", 
	year={1991}, 
	month={September}, 
	volume={37}, 
	number={5}, 
	pages={1412-1418}
}

@Article{wu_icl14,
  author  = {Daolong Wu and Ying Li and Yue Sun},
  title   = {{Construction and block error rate analysis of polar codes over AWGN channel based on Gaussian approximation}},
  journal = {IEEE Commun. Lett.},
  year    = {2014},
  volume  = {18},
  number  = {7},
  pages   = {1099-1102},
  month   = jul,
}

@Article{X.N_08,
  author =  {X. Ningde and X. Wei and Z. Tong and E. F. Haratsch and M. Jaekyun},
  title =   {{Concatenated low-density parity-check and BCH coding system for magnetic recording read channel with 4 kb sector format}},
  journal = {IEEE Transactions on Magnetics},
  year =    {2008},
  volume =  {44},
  number =  {12},
  pages =   {4784-4789}
}
@misc{xia_13,
  author = {Venkatesan Guruswami and Patrick Xia},
  title = "{Polar Codes: Speed of Polarization
and Polynomial Gap to Capacity}",
  howpublished = "\url{http://arxiv.org/abs/1304.4321}",
  year = {2013}, 
  note = {``[Submitted on 16 Apr 2013]''},
}
@article{xu_jsac06,
	author = "Zhengyuan Xu and B. M. Sadler",
	title = "{Multiuser Transmitted Reference Ultra-Wideband Communication Systems}",
	journal = "{IEEE Journal on Selected Areas in Communications}",
	volume = 24,
	number = 4,
	pages = "766-772",
	month = "Apr.",
	year = "2006"
	}

@InProceedings{ya_vtc16,
  author    = {Ya Meng and Liping Li and Yanjun Hu},
  title     = {{A novel interleaving scheme for polar codes}},
  booktitle = {Proc. IEEE Veh. Technol. Conf. Fall (VTC-Fall)},
  year      = {2016},
  pages     = {1-5},
  month     = sep,
}

@Book{yeh_06,
  title =     {{Real analysis: Theory of measure and integration}},
  publisher = {World Scientific Publishing Co.},
  year =      {2006},
  author =    {J Yeh},
  edition =   {2nd}
}

@Misc{mackay_02,
  author       = {David J.C. Mackay},
  title        = {{Good error-correcting codes based on very sparse matrices}},
  howpublished = {[Online]. Available: \url{http://www.inference.phy.cam.ac.uk/mackay/CodesGallager.html}},
  month        = jul,
  year         = {2002},
}

@Article{Stefan_infoTheory02,
  author = {Stefan H\"ost, Rolf Johannesson, and Victor V. Zyablov},
  title  = {Woven Convolutional Codes I: Encoder Properties},
  year   = {2002},
  volume = {48},
  number = {1},
  pages  = {149-161},
  month  = jan,
}

@Comment{jabref-meta: databaseType:bibtex;}

